On Transferability of Prompt Tuning for Natural Language Processing

Prompt tuning (PT) is a promising parameter-efficient method to utilize extremely large pre-trained language models (PLMs), which can achieve comparable performance to full-parameter fine-tuning by only tuning a few soft prompts. However, PT requires much more training time than fine-tuning. Intuitively, knowledge transfer can help to improve the efficiency. To explore whether we can improve PT via prompt transfer, we empirically investigate the transferability of soft prompts across different downstream tasks and PLMs in this work. We find that (1) in zero-shot setting, trained soft prompts can effectively transfer to similar tasks on the same PLM and also to other PLMs with a cross-model projector trained on similar tasks; (2) when used as initialization, trained soft prompts of similar tasks and projected prompts of other PLMs can significantly accelerate training and also improve the performance of PT. Moreover, to explore what decides prompt transferability, we investigate various transferability indicators and find that the overlapping rate of activated neurons strongly reflects the transferability, which suggests how the prompts stimulate PLMs is essential. Our findings show that prompt transfer is promising for improving PT, and further research shall focus more on prompts' stimulation to PLMs. The source code can be obtained from https://github.com/thunlp/Prompt-Transferability.

==> revise.tex <==

- Check:
4. prompt transfer or prompt transferred (unify)

5. propose: task similarity (task)
6. Name transferability 
7. help to + V ==> help + V


==========
(Intrics exps)
Model-level effectiveness: explore the intrics dim (from 10 to 100)
- less parameters

- When target is few shot settings 
- Transfer the same prompts to the same tasks (and avg)

====================================
====================================
-Task transfer (實驗可看performance和convergence speed)，但不是重點。
-重點是 激活模型參數 可以用來良好度量prompt 相似度

- 增強 "激活模型參數 可以用來良好度量prompt 相似度" 結論，對prompt加入擾動，測量cos, enc和activated neurons.




==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph{Using multiple source prompts.}
In both \TPTtask and \TPTmodel, we only use one source prompt for initialization, which is a prior attempt. Intuitively, mixing up multiple source prompts may achieve further performance and efficiency gain. Actually, concurrent work~\citep{vu2021spot} has confirmed this in the cross-task transfer. Future work can explore advanced mixing/ensemble methods for better initialization, and the explored prompt similarity metrics in this paper may help to this end.


\paragraph{Finding better prompt similarity metric.}
In \cref{ssec:transferring_with_initialization_cross-model}, we find that although the prompts projected from another PLM can achieve comparable performance to prompts originally trained on the target PLM, these two kinds of prompts are highly dissimilar when measured by all the prompt similarity metrics in this paper, including the overlapping rate of activated neurons. This shows that we still need a better prompt similarity metric considering the high redundancy of PLMs and measuring the essential factors of prompts, which needs a deeper understanding on the mechanisms of PLMs.
Previous works~\citep{Aghajanyan2021IntrinsicDE,qin2021exploring} show that various NLP tasks can be reparameterized into similar low-dimensional subspaces conditioning on PLMs, which may help to this end. 


\paragraph{Designing better cross-model prompt projection.}
Compared with \TPTtask, the results of \TPTmodel in this paper are much weaker due to the different characteristics between source and target PLMs and the limited projection methods. In \cref{ssec:transferring_with_initialization_cross-model}, we find our cross-model projection tends to project into the solutions of comparable performance but not those preferred by the optimization process; thus \TPTmodel works not as well as \TPTtask. And we find that when we remove the $\mathrm{LayerNorm}(\cdot)$ of Eq.~\ref{eq:transfer_projector} in \textbf{Task Tuning}, this phenomenon is even more significant that the learning loss does not decrease when using \TPTmodel. For the details, please refer to \cref{ssec:appendix_initialization_experiments_cross-model}. This suggest that we should design better cross-model projection methods to overcome the heterogeneity of different PLMs and different optimization preferences.

==> sections/experiment_settings.tex <==
\begin{table*}[!htbp]
\begin{center} 
%\small
\scalebox{0.8}
{
{
\setlength\tabcolsep{0.35em}
\begin{tabular}{l|cccccc|ccc|cc|cc}
\toprule
  \multicolumn{1}{c|}{\textbf{Task Type}} & \multicolumn{6}{c|}{\textbf{Sentiment Analysis (SA)}} & \multicolumn{3}{c|}{\textbf{NLI (NLI)}} & \multicolumn{2}{c|}{\textbf{Ethics Judgment (EJ)}} & \multicolumn{2}{c}{\textbf{\makecell[c]{Paraphrase\\Identification (PI)}}}
  \\
  \midrule
  {\textbf{Prompt}} & {IMDB} & {SST-2} & {laptop} & {\makecell[c]{resta\\-urant}} & {Movie} & {Tweet} & {MNLI} & {QNLI} & {SNLI} & {\makecell[c]{deonto\\-logy}} & {justice} & {QQP} & {MPRC} \\
\midrule
{\textbf{Labels}} & {$2$} & {$2$} & {$4$} & {$4$} & {$2$} & {$3$} & {$3$} & {$2$} & {$3$} & {$2$} & {$2$} & {$2$} & {$2$} \\
{\textbf{Std.(\%)}} & {$0.1$} & {$0.5$} & {$0.9$} & {$0.6$} & {$0.2$} & {$0.2$} & {$0.5$} & {$0.1$} & {$0.3$} & {$0.4$} & {$0.4$} & {$0.1$} & {$0.7$} \\
{\textbf{Acc.(\%)}} & {$89.7$} & {$93.3$} & {$75.3$} & {$79.5$} & {$76.0$} & {$74.5$} & {$83.1$} & {$90.5$} & {$88.5$} & {$71.7$} & {$67.8$} & {$86.9$} & {$84.4$} \\
\bottomrule
\end{tabular}}}
\caption{Acc.(\%) and Std.(\%) of tuned soft prompts underlying \RoBERTaBASE on $13$ NLU tasks.}
\label{table:soft_prompts_performance}
\end{center} 
\end{table*}











% \section{Experiment Settings}
% \label{sec:experiment_settings}
% We first describe the evaluated tasks and the corresponding datasets we used in this paper in \cref{ssec:task_and_dataset}. Then we introduce the implementation details for soft prompt tuning in \cref{ssec:Soft_prompt_tuning_setting}. As mentioned before, we focus on both cross-task and cross-model soft prompt transfer, and we investigate whether the source prompts (1) would have satisfying zero-shot performance on target tasks / models, and (2) could serve as good initialization for further optimization.

%Besides, we demonstrate that the overlapping percentage of activated parameters is a better metric to measure similarities between prompts. Finally, we introduce a transfer projector to better transfer source prompt to target PLMs. 


\subsection{Task and Dataset}
\label{ssec:task_and_dataset}
In this paper, we mainly focus on natural language understanding (NLU) tasks and choose $4$ representative categories: (1) Emotion Classification~(Emotion), including IMDB~\cite{maas-EtAl:2011:ACL-HLT2011}, SST-2~\cite{socher-etal-2013-recursive}, laptop~\cite{pontiki-etal-2014-semeval}, restaurant \cite{pontiki-etal-2014-semeval}, Movie Rationales(Movie) \cite{zaidan-eisner-piatko-2008:nips} and TweetEval(Tweet) \cite{barbieri-etal-2020-Tweeteval}, (2) Natural Language Inference~(NLI), including MNLI \cite{williams-etal-2018-broad}, QNLI \cite{wang2018glue} and SNLI \cite{bowman-etal-2015-large}, (3) Ethical Acceptability~(Ethics), including deontology \cite{hendrycks2021aligning} and justice \cite{hendrycks2021aligning}, and (4) Semantics Similarity~(Semantics), including QQP \cite{sharma2019natural}, and MRPC \cite{dolan-brockett-2005-automatically}. More details about these datasets are left in the appendix.

% We exploit IMDB~\cite{maas-EtAl:2011:ACL-HLT2011}, SST-2~\cite{socher-etal-2013-recursive}, laptop~\cite{pontiki-etal-2014-semeval}, restaurant \cite{pontiki-etal-2014-semeval}, Movie Rationales(Movie) \cite{zaidan-eisner-piatko-2008:nips}, TweetEval(Tweet) \cite{barbieri-etal-2020-Tweeteval}, MNLI \cite{williams-etal-2018-broad}, QNLI \cite{wang2018glue}, SNLI \cite{bowman-etal-2015-large}, deontology \cite{hendrycks2021aligning}, justice \cite{hendrycks2021aligning}, QQP \cite{sharma2019natural}, and MRPC \cite{dolan-brockett-2005-automatically} datasets. These datasets include $4$ types of NLU tasks: Emotion Classification~(Emotion), Natural Language Inference~(NLI), Ethical Acceptability~(Ethics), and Semantics Similarity~(Semantics). Readers can refer to the appendix for more detail about these datasets and tasks. 



\subsection{Training Details for Soft Prompt Tuning}
\label{ssec:Soft_prompt_tuning_setting}
We choose \BertBASE~\cite{devlin-etal-2019-bert}, \RoBERTaBASE and \RoBERTaLARGE~\cite{liu2019roberta} as the main evaluated PLMs. We set the length $l$ of the soft prompt tokens to $100$, and replace the first token with $\mathtt{[MASK]}$, where embedding is frozen during the prompt tuning.

% prepend a frozen $\mathtt{[MASK]}$ token and the soft prompts before the original input $\{x_1,\ldots,x_n\}$. 

% the first position is the \texttt{[mask]} whose embedding is initialized with itself and frozen during the tuning. The dimension $d$ of each newly added token is $768$, which is consistent with the \RoBERTaBASE's embedding dimension.
Besides, we do not add the position embedding or the type embedding into the prompt during the prompt tuning. All the soft prompts are randomly initialized, and optimized with Equation \ref{eq:continuous_prompt_tuning}. For those tasks corresponding to the same type, their labels are mapped to the same set of target tokens by the verbalizer.
% same-type tasks corresponds to the same label verbalizer sets but each of them may use different numbers of verbalizers. Reader can refer to Appendix \cref{sec:appendix} for more detail about used verbalizers.
% For evaluation, we respectively report task mean performance with three different random seeds and standard deviations as show in Table~\ref{table:soft_prompts_performance}. 

%In the following experiments, we will use PT by this setting to tuned prompts.


%with three different $3$ random seeds

% we will study the following questions and exploit these tuned prompts to verify the transferability in every setting.




% \subsection{Cross-Domain}
% \label{ssec:cross-domain}
% \subsubsection{Cross-Domain Performance}
% \label{sssec:cross_domain_performance}
% We choose emotion classification and NLI tasks for the cross-domain experiment. For emotion classification task, we re-tune prompts on the instances with positive and negative labels. For NLI task, we re-tune prompts on the instances with entailment and contradiction labels. Except for the domains, we freeze other control variables, which meets the experiment settings better.
% \paragraph{Setting} Transfer source prompts to the same task underlying different domains to verify the performances. 
% \paragraph{Approach} Directly re-use source prompts.
% \paragraph{Analysis} In the evaluation stage, we valid the prompts with the same number of target domain instances hybridizing different percentage target and source domain instances. As the increasing percentage of source domain instances, the performances become better in Figure~\ref{fig:domain}.



% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=1\textwidth]{figs/task_transferability_result.pdf}
% \caption{When the source and target tasks are similar, the source prompt can benefit the target tasks. The shade of color shows the transferability for source prompts to target tasks.}
% \label{fig:task_transferability_result}
% \end{figure*}






% \begin{table*}[!htbp]
% \begin{center} 
% %\small
% \scalebox{0.8}
% {
% {
% \setlength\tabcolsep{0.25em}
% \begin{tabular}{l|cccccc|cccc|cc|cc|c}
% \toprule
%   \multicolumn{1}{c|}{\textbf{Correlation}} & \multicolumn{6}{c|}{\textbf{Emotion}} & \multicolumn{4}{c|}{\textbf{NLI}} & \multicolumn{2}{c|}{\textbf{Ethics}} & \multicolumn{2}{c|}{\textbf{Semantics}} & \multicolumn{1}{c}{\textbf{Overall}}
%   \\
%   \midrule
%   {\textbf{Metrics}} & {IMDB} & {SST-2	} & {laptop} & {\makecell[c]{resta\\-urant}} & {Movie} & {Tweet} & {MNLI} & {QNLI} & {SNLI} & {ner} & {\makecell[c]{deonto\\-logy}} & {justice} & {QQP} & {MPRC} & {Overall} \\
% \midrule
% {{$\mathrm{S}_{\texttt{overlap}}$}} & {\textbf{95.3}} & {95.9} & {\textbf{97.4}} & {\textbf{96.6}} & {\textbf{92.7}} & {\textbf{97.6}} & {\textbf{98.7}} & {\textbf{98.0}} & {\textbf{98.5}} & \textbf{{91.5}} & \textbf{{91.9}} & \textbf{{90.7}} & {93.8} & \textbf{{90.1}} & \textbf{{94.9}} \\
% {{Euclidean}} & {90.7} & {\textbf{97.2}} & {79.3} & {83.2} & {64.1} & {96.2} & {97.5} & {97.3} & {97.8} & {89.6} & {81.0} & {76.6} & \textbf{{97.6}} & {68.3} & {86.9} \\
% \bottomrule
% \end{tabular}}}
% \caption{By measuring similarity between prompts with overlapping percentages of activated parameters ($\mathrm{S}_{\texttt{overlap}}$) and Euclidean distance (Euclidean), we find that $\mathrm{S}_{\texttt{overlap}}$ scores have higher correlations (\%) with the performances of transferred prompts, namely ($\mathrm{S}_{\texttt{overlap}}$) can better measure prompt similarities.}
% \label{table:prompt_similiarty_measure}
% \end{center} 
% \end{table*}





% \begin{figure}[!htb]
%     \centering
%     % \subfigure[IMDB training loss.]{
%     %     \includegraphics[width=0.225\textwidth]{figs/IMDB_train_loss.pdf}
%     % }
%     % \subfigure[IMDB eval Acc.]{
%     % 	\includegraphics[width=0.225\textwidth]{figs/IMDB_eval_acc.pdf}
%     % }
%     \subfigure[MNLI training loss.]{
% 	    \includegraphics[width=0.225\textwidth]{figs/MNLI_train_loss.pdf}
%     }
%     \subfigure[MNLI eval Acc.]{
% 	    \includegraphics[width=0.225\textwidth]{figs/MNLI_eval_acc.pdf}
%     }
%     \subfigure[Deontology training loss.]{
% 	    \includegraphics[width=0.225\textwidth]{figs/deont_train_loss.pdf}
%     }
%     \subfigure[Deontology eval Acc.]{
% 	    \includegraphics[width=0.225\textwidth]{figs/deont_eval_acc.pdf}
%     }
%     \caption{Utilizing source prompts from similar tasks as initialization for prompt tuning (\textcolor{orange}{\textemdash}) has faster convergence and sometimes achieves better performance than prompt tuning from scratch (\textcolor{blue}{\textemdash}).}
%     \label{fig:transfer_task_coverage}
% \end{figure}





% \begin{figure}[!htb]
% \centering
% \includegraphics[width=0.48\textwidth]{figs/task_activate_layers.pdf}
% \caption{We calculate overlapping percentages of activated parameters between prompts in 1-2 layers, 12 layers, and 11-12 layers of a PLM and average the overlapping percentages by the task types (Emotion, NLI, Ethics, Semantics). With the increasing depth of layers, the overlapping percentage decreases, namely the prompts activated more task-specific parameters in deeper layers.}
% \label{fig:activaed_parameters_in_different_layers}
% \end{figure}



% \subsection{Cross-Task}
% \label{ssec:cross-task}
% \subsubsection{Cross-task Performance}
% \label{sssec:cross_task_performance}
% \paragraph{Setting} Transfer source prompts to various target tasks
% \paragraph{Approach} Directly re-use source prompts.
% \paragraph{Analysis} As shown in Figure~\ref{fig:task_transferability_result}, we transfer source prompts to various target tasks. When target tasks are similar to source tasks, the source prompts can achieve better performances on them.



% \subsubsection{Cross-Task Prompt Similarity}
% \label{sssec:cross-task_prompt_similarity}
% \paragraph{Setting} Measure the similarities among prompts underlying the same PLM.
% \paragraph{Approach} (1) Calculate Euclidean distances in embedding space between two source prompts (2) Calculate the similarity between prompts with overlapping activated parameters in the PLM as we introduce in Section~\ref{ssec:overlapping_percentage_of_activated parameters}.

% \paragraph{Analysis} By respectively calculating Euclidean distances and overlapping percentages of activated parameters in Equation~\ref{eq:overlap_ap}, we find that exploiting overlapping percentages as show in Figure~\ref{fig:task_overlap_12_layers_half} can better present prompts similarity than using Euclidean distances~\ref{fig:task_euclidean_half}.

% By comparing the euclidean distance in Figure~\ref{fig:task_euclidean_half} and the transferability result in Figure~\ref{fig:task_transferability_result}, we find that the close prompts in embedding space cannot benefit each other after transferring to each other's tasks, which means euclidean distances may not clearly measure transferabilies for prompts.

% On the other hand, overlapping percentages as show in Figure~\ref{fig:task_overlap_12_layers_half} can better determine whether two prompts can transfer to each other's tasks in Figure~\ref{fig:task_transferability_result}, which means it can better measure similarities between prompts.

% Furthermore, we take a further step to explore the overlapping percentages in different depth of layers and find that prompts are gradually prone to activating task-specific parameters with the increasing depth of layers for the PLM. Thus, as show in Figure~\ref{fig:activaed_parameters_in_different_layers}, the overlapping percentages of activated parameters will not only decrease between two different tasks but also demonstrate the same taks underlying different datasets. Readers can refer to Appendix~\ref{sec:appendix} where we comprehensively visualized the overlapping percentages of activated parameters on the upper and lower layers for prompts underlying \RoBERTaBASE.

% According to the above conclusions, the overlapping percentage of activated parameters is more suitable to measure the similarity for a pair of prompts instead of directly using the Euclidean distance between prompts.




% \subsubsection{Cross-Task Initialization}
% \label{sssec:cross_task_initialization}
% \paragraph{Setting} Conduct prompt tuning for target tasks with the initializations of source prompts.
% \paragraph{Approach} Directly reuse source prompts as the initializations.
% \paragraph{Analysis} Among these 14 datasets~\ref{ssec:task_and_dataset}, we choose MNLI and Deontology for initialization experiments due to their slow converge during prompt tuning. By leveraging source prompts as initialization for similar target tasks to perform soft prompt tuning, the target prompts have faster converge than tuning from scratch as shown in Figure~\ref{fig:transfer_task_coverage}. Cross-domain initialization can mitigate slow converge during tuning to some degree.







% \begin{table*}[!htb]
% \begin{center} 
% %\small
% \scalebox{0.8}
% {
% {
% \setlength\tabcolsep{0.25em}
% \begin{tabular}{l|cccccc|cccc|cc|cc}
% \toprule
%   \multicolumn{15}{c}{\BertBASE to \RoBERTaBASE (Acc.\%)} \\
%   \midrule
%   \multicolumn{1}{c|}{\textbf{Task}} & \multicolumn{6}{c|}{\textbf{Emotion}} & \multicolumn{4}{c|}{\textbf{NLI}} & \multicolumn{2}{c|}{\textbf{Ethics}} & \multicolumn{2}{c}{\textbf{Semantics}}
%   \\
%   \midrule
%   {\textbf{Dataset}} & {IMDB} & {SST-2	} & {laptop} & {\makecell[c]{resta\\-urant}} & {Movie} & {Tweet} & {MNLI} & {QNLI} & {SNLI} & {ner} & {\makecell[c]{deonto\\-logy}} & {justice} & {QQP} & {MPRC} \\
% \midrule
% PT (on \BertBASE) & 50.3 & 51.0 & 2.5 & 41.5 & 49.5 & 40.8 & 32.4 & 50.6 &  31.5 & 50.0 & 50.3 & 50.0 & 36.8 & 68.0 \\ 
% \midrule
% PT (on \RoBERTaBASE) & 89.7 & 93.3 & 75.3 & 79.5 & 76.0 & 74.5 & 79.9 & 90.5 & 88.5 & 94.9 & 71.7 & 67.8 & 86.9 & 84.4 \\
% \midrule
% \midrule
% Projector (random) & 51.3 & 52.4 & 10.6 & 1.30 & 50.5 & 40.9 & 31.7 & 50.6 & 33.4 & 50.0 & 50.4 & 50.0 & 38.7 & 69.3 \\
% \midrule
% \multicolumn{15}{c}{Embedding Projector} \\
% \midrule
% $\mathbf{Proj}_{e}$ (IMDB,laptop) & {89.7} & {64.4} & {75.6} & {21.6} & {53.1} & {30.1} & {33.6} & {51.6} &  {33.4} & {50.1} & {51.0} & {51.2} & {48.7} & {48.7} \\ 
% $\mathbf{Proj}_{e}$ (MNLI) & {50.4} & {51.2} & {51.9} & {63.6} & {50.5} & {41.0} & {80.0} & {50.6} &  {33.3} & {50.0} & {50.4} & {49.9} & {36.8} & {53.7} \\ 
% $\mathbf{Proj}_{e}$ (all) & {56.5} & {92.9} & {36.1} & {56.9} & {50.5} & {72.1} & {79.8} & {90.8} &  {88.4} & {94.7} & {50.4} & {50.2} & {86.9} & {33.3} \\ 
% \midrule
% \multicolumn{15}{c}{Prompt Tuning Projector} \\
% \midrule
% $\mathbf{Proj}_{pt}$ (IMDB,laptop) & 86.5 & 84.9 & 73.4 & 75.3 & 76.6 & 47.7 & 31.8 & 52.0 & 32.9 & 50.0 & 50.3 & 50.0 & 37.6 & 67.5 \\
% $\mathbf{Proj}_{pt}$ (MNLI) & 66.6 & 70.4 & 53.0 & 43.8 & 57.8 & 47.9 & 82.4 & 74.9 & 78.1 & 60.4 & 50.4 & 49.9 & 45.3 & 70.1 \\
% $\mathbf{Proj}_{pt}$ (all) & 88.4 & 91.2 & 76.1 & 82.5 & 76.0 & 51.9 & 55.2 & 79.5 & 69.8 & 90.5 & 50.4 & 50.0 & 70.6 & 88.0 \\
% \bottomrule
% \end{tabular}}}
% \caption{We can transfer a source prompt from \BertBASE to \RoBERTaBASE by well-trained $\mathbf{Proj}_{pt}$. The projector even can generalize to unseen but similar tasks.}
% \label{table:bertbase_to_robertabase}
% \end{center} 
% \end{table*}







% \begin{table*}[!htb]
% \begin{center} 
% %\small
% \scalebox{0.8}
% {
% {
% \setlength\tabcolsep{0.25em}
% \begin{tabular}{l|cccccc|cccc|cc|cc}
% \toprule
%   \multicolumn{15}{c}{\RoBERTaBASE to \RoBERTaLARGE (Acc.\%)} \\
%   \midrule
%   \multicolumn{1}{c|}{\textbf{Task}} & \multicolumn{6}{c|}{\textbf{Emotion}} & \multicolumn{4}{c|}{\textbf{NLI}} & \multicolumn{2}{c|}{\textbf{Ethics}} & \multicolumn{2}{c}{\textbf{Semantics}}
%   \\
%   \midrule
%   {\textbf{Dataset}} & {IMDB} & {SST-2} & {laptop} & {\makecell[c]{resta\\-urant}} & {Movie} & {Tweet} & {MNLI} & {QNLI} & {SNLI} & {ner} & {\makecell[c]{deonto\\-logy}} & {justice} & {QQP} & {MPRC} \\
% \midrule
% Target (\RoBERTaLARGE) & 91.8 & 94.6 & 78.1 & 81.7 & {81.7} & 76.6 & 88.5 & 93.4 & 90.7 & {95.53} & {85.6} & {81.1} & 89.0 & 82.7 \\
% \midrule
% \midrule
% Projector (random) & 50.3 & 51.0 & 48.6 & 39.1 & 52.6 & 35.2 & 34.3 & 51.4 & 33.6 & 50.1 & 50.3 & 50.0 & 51.35 & 55.3 \\
% \midrule
% Projector (Token Emb.) & {49.7} & {54.2} & {17.2} & {8.7} & {49.0} & {42.0} & {33.1} & {50.4} &  {33.1} & {50.0} & {50.3} & {50.1} & {37.2} & {58.4} \\ 
% \midrule
% \multicolumn{15}{c}{Embedding Projector} \\
% \midrule
% $\mathbf{Proj}_{e}$ (IMDB,laptop) & {92.0} & {50.5} & {76.6} & {14.8} & {53.1} & {41.0} & {32.9} & {51.0} &  {33.3} & {50.0} & {50.3} & {49.7} & {52.8} & {51.6} \\ 
% $\mathbf{Proj}_{e}$ (MNLI) & {50.4} & {50.5} & {46.8} & {45.5} & {49.0} & {41.2} & {88.5} & {49.8} &  {31.6} & {50.5} & {50.3} & {49.7} & {36.9} & {67.2} \\ 
% $\mathbf{Proj}_{e}$ (all) & {} & {} & {} & {} & {} & {} & {} & {} &  {} & {} & {} & {} & {} & {} \\ 
% \midrule
% \multicolumn{15}{c}{Prompt Tuning Projector} \\
% \midrule
% $\mathbf{Proj}_{pt}$ (IMDB+laptop) & 90.4 & 76.2 & 64.2 & 69.5 & 79.7 & 45 & 33.3 & 50.5 & 33.1 & 50.0 & 50.3 & 50.0 & 38.5 & 79.7 \\
% $\mathbf{Proj}_{pt}$ (MNLI) & 67.7 & 76.1 & 28.9 & 43.7 & 60.4 & 49.1 & 87.1 & 79.4 & 84.5 & 63.9 & 49.7 & 50.0 & 36.8 & 68.5 \\
% $\mathbf{Proj}_{pt}$ (all) & 77.3 & 79.7 & 66.6 & 73.6 & 65.1 & 46.5 & 44.4 & 57.1 & 40.0 & 59.5 & 50.4 & 50.0 & 69.2 & 73.7 \\
% \bottomrule
% \end{tabular}}}
% \caption{We can transfer a source prompt from \RoBERTaBASE to \RoBERTaLARGE by well-trained $\mathbf{Proj}_{pt}$. The projector even can generalize to unseen but similar tasks.}
% \label{table:robertabase_to_robertalarge}
% \end{center} 
% \end{table*}













% \begin{figure*}[!htb]
% \subcapraggedrighttrue
% \subcaphangtrue
%     \centering
%     \subfigure[MNLI training loss. \texttt{[Base to Large]}]{
% 	    \includegraphics[width=0.225\textwidth]{figs/MNLI_train_loss_base_large.pdf}
%     }
%     \subfigure[MNLI training loss. \texttt{[Bert to Roberta]}]{
% 	    \includegraphics[width=0.225\textwidth]{figs/MNLI_train_loss_bert_roberta.pdf}
%     }
%     \subfigure[IMDB training loss. \texttt{[Base to Large]}]{
% 	    \includegraphics[width=0.225\textwidth]{figs/IMDB_train_loss_base_large.pdf}
%     }
%     \subfigure[IMDB training loss. \texttt{[Bert to Roberta]}]{
% 	    \includegraphics[width=0.225\textwidth]{figs/IMDB_train_loss_bert_roberta.pdf}
%     }
%     \subfigure[MNLI eval Acc. ~~~~\texttt{[Base to Large]}]{
% 	    \includegraphics[width=0.225\textwidth]{figs/MNLI_eval_acc_base_large.pdf}
%     }
%     \subfigure[MNLI eval Acc. ~~~~\texttt{[Bert to Roberta]}]{
% 	    \includegraphics[width=0.225\textwidth]{figs/MNLI_eval_acc_bert_roberta.pdf}
%     }
%     \subfigure[IMDB eval Acc. ~~~\texttt{[Base to Large]}]{
% 	    \includegraphics[width=0.225\textwidth]{figs/IMDB_eval_acc_base_large.pdf}
%     }
%     \subfigure[IMDB eval Acc. ~~~\texttt{[Bert to Roberta]}]{
% 	    \includegraphics[width=0.225\textwidth]{figs/IMDB_eval_acc_bert_roberta.pdf}
%     }
%     \caption{Utilizing projected prompts from the same tasks as initialization to perform prompt tuning on the target PLM (\textcolor{orange}{\textemdash}) cannot speed up the convergence and is even stuck into a local minimize point, which performs worse than prompt tuning from scratch (\textcolor{blue}{\textemdash}).}
%     \label{fig:transfer_model_coverage}
% \end{figure*}







% \begin{table*}[!htb]
% \begin{center} 
% %\small
% \scalebox{0.725}
% {
% {
% \setlength\tabcolsep{0.22em}
% \begin{tabular}{l|ccccc}
% \toprule
%   \multicolumn{6}{c}{Similarity Between Prompts} \\
%   \midrule
%   \multicolumn{1}{c|}{\textbf{Task}} & \multicolumn{3}{c|}{\textbf{Emotion}} &
%   \multicolumn{2}{c}{\textbf{NLI}}  
%   \\
%   \midrule
%   \multicolumn{1}{c|}{\textbf{Prompt}} & {IMDB} & {laptop} & \multicolumn{1}{c|}{\makecell[c]{resta\\-urant}} & \multicolumn{1}{c|}{MNLI} & \multicolumn{1}{c}{SNLI} \\
% \midrule
% \midrule
% \multicolumn{6}{c}{Overlapping Parameters}\\
% \midrule
% \multicolumn{1}{c|}{MNLI (target)} & \multicolumn{1}{c}{0.14} & \multicolumn{1}{c}{0.12} & \multicolumn{1}{c|}{0.16} & \multicolumn{1}{c}{1.00} & \multicolumn{1}{c}{0.43} \\
% \multicolumn{1}{c|}{MNLI ($\mathbf{Proj}_{pt}$(MNLI))} & \multicolumn{1}{c}{0.11} & \multicolumn{1}{c}{0.16} & \multicolumn{1}{c|}{0.16} & \multicolumn{1}{c}{0.21} & \multicolumn{1}{c}{0.25} \\ 
% \midrule
% \multicolumn{1}{c|}{IMDB (target)} & \multicolumn{1}{c}{1.00} & \multicolumn{1}{c}{0.32} & \multicolumn{1}{c|}{0.32} & \multicolumn{1}{c}{0.14} & \multicolumn{1}{c}{0.19} \\ 
% \multicolumn{1}{c|}{{IMDB ($\mathbf{Proj}_{pt}$(IMDB,laptop))}} & \multicolumn{1}{c}{0.37} & \multicolumn{1}{c}{0.36} & \multicolumn{1}{c|}{0.36} & \multicolumn{1}{c}{0.17} & \multicolumn{1}{c}{0.18} \\
% \midrule
% \multicolumn{6}{c}{Enculidance Distance} \\
% \midrule
% \multicolumn{1}{c|}{MNLI (target)} & \multicolumn{1}{c}{71709} & \multicolumn{1}{c}{71187} & \multicolumn{1}{c|}{71245} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{97381}\\
% \multicolumn{1}{c|}{MNLI ($\mathbf{Proj}_{pt}$(MNLI))} & \multicolumn{1}{c}{6553635127296} & \multicolumn{1}{c}{6553635127296} & \multicolumn{1}{c|}{6553635127296} & \multicolumn{1}{c}{6553635127296} & \multicolumn{1}{c}{6553635127296}\\ 
% \midrule
% \multicolumn{1}{c|}{IMDB (target)} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{10780} & \multicolumn{1}{c|}{11153} & \multicolumn{1}{c}{71709} & \multicolumn{1}{c}{68729}\\ 
% \multicolumn{1}{c|}{{IMDB ($\mathbf{Proj}_{pt}$(IMDB,laptop))}} & \multicolumn{1}{c}{1608447232} & \multicolumn{1}{c}{1608447616} & \multicolumn{1}{c|}{1608447616} & \multicolumn{1}{c}{1608446976} & \multicolumn{1}{c}{1608445184} \\
% \bottomrule
% \end{tabular}}}
% \caption{Measure similarities between projected prompts and prompt-tuned prompts with the enculidance distance and the overlapping percentages of activated parameters, we find that overlapping percentages can better present the similarities.}
% \label{table:projected_prompt_enculidance_distances_and_overlapping_percentage}
% \end{center} 
% \end{table*}


% \subsection{Cross-Model}
% \label{ssec:cross-model}

% \subsubsection{Cross-Model Performance}
% \label{sssec:cross-model_performance}
% \paragraph{Setting} Transfer prompts to heterogeneous target PLMs, which are different types or sizes of PLM. Specifically, (1) we transfer source prompts on \BertBASE to \RoBERTaBASE; (2) we transfer source prompts on \RoBERTaBASE to \RoBERTaLARGE.
% \paragraph{Approach} We leverage two different transfer projectors, the embedding projector and the prompt tuning projector, as we introduce in Section~\ref{ssec:transfer_projector}.
% \paragraph{Analysis} 
% As clearly shown in Table~\ref{table:bertbase_to_robertabase}, directly applying source prompts to target PLMs for the same tasks does not work, not to mention the inconsistent dimension size between source and target PLMs.

% To transfer source prompts to target PLMs, we attempt to design the embedding projector to transfer source prompts to the target PLMs. The embedding projector can successfully transfer source prompts of seen tasks in the stage of training the projector. However, the embedding projector seems to be specific for tasks seen in the projector training stage. 

% We take a further step to replace the embedding projector with the prompt tuning projector. In the same settings, the prompt tuning projector not only can achieve good performances on seen tasks but generalize to similar tasks as shown in Table~\ref{table:bertbase_to_robertabase} and Table~\ref{table:robertabase_to_robertalarge}.

% According to the cross-model performance results, the prompt tuning projector is the better method for the cross-model transfer. 



% \subsubsection{Cross-Model Prompt Similarity}
% \label{sssec:cross-task_prompt_similarity}
% \paragraph{Setting} Measure the similarities between projected prompts transferred with $\mathbf{Proj_{pt}(\cdot)}$ and targets prompts trained from scratch by prompt tuning (PT).

% \paragraph{Approach} (1) Calculate Euclidean distances in embedding space between two projected and targets prompts (2) Calculate the similarity between projected and targets prompts with overlapping activated parameters in the target PLM as we introduce in Section~\ref{ssec:overlapping_percentage_of_activated parameters}.

% \paragraph{Analysis} By leveraging $\mathbf{Proj_{pt}(\cdot)}$, we can obtain comparable performances with those target prompts tuned on the target tasks from scratch. Interestingly, while these projected and target prompts have comparable performances on the same tasks, they are far away from each other with enculidance distances. Overlapping parameters for the target common PLMs can better present the functions between prompts as show in Table~\ref{table:bertbase_to_robertabase}. Thus, again, the overlapping percentage of activated parameters may be the better method to measure similarity for prompts. Besides, another interesting finding is that $\mathbf{Proj_{pt}(\cdot)}$ may find another prompt for the specific tasks.


% \subsubsection{Cross-Model Initialization}
% \label{sssec:cross-model_initialization}
% \paragraph{Setting} Compare prompt tuning coverage speeds between using or not using corresponding projected prompts as initialization.
% \paragraph{Approach} Using projected prompts as the initialization for the corresponding tasks.
% \paragraph{Analysis} We repseitively choose MNLI and IMDB datasets for this experiments, since projected prompts of MNLI and IMDB can achieve compare performances with prompt tuning on target PLMs. These prompts cannot benefit prompt tuning to speed up the coverage, which may be stuck on local minimize points. 


% In cross-domain experiments, we not only propose a projector to transfer prompts but surprisedly find multiple prompts can achieve comparable performances with each other. Namely, these multiple prompts may be consistent for a common PLM, and we can leverage overlapping percentages of activated parameters to claim these prompts are highly similar. Thus, again, this demonstrates that overlapping percentages can better measure similarities between prompts.

